Measurement of prompt D$^0$, D$^+$, D$^{*+}$, and D$^+_s$ production in p-Pb collisions at $\sqrt{s_{\rm{NN}}}$ = 5.02 TeV

The measurement of the production of prompt D$^0$, D$^+$, D$^{*+}$, and D$^+_s$ mesons in proton$-$lead (p$-$Pb) collisions at the centre-of-mass energy per nucleon pair of $\sqrt{s_{\rm NN}}$ = 5.02 TeV, with an integrated luminosity of $292\pm 11$ $\mu$b$^{-1}$, are reported. Differential production cross sections are measured at mid-rapidity ($-0.96<y_{\rm cms}<0.04$) as a function of transverse momentum ($p_{\rm T}$) in the intervals $0< p_{\rm T} < 36$ GeV/$c$ for D$^0$, $1< p_{\rm T} <36$ GeV/$c$ for D$^+$ and D$^{*+}$, and $2< p_{\rm T} <24$ GeV/$c$ for D$^+_s$ mesons. For each species, the nuclear modification factor $R_{\rm pPb}$ is calculated as a function of $p_{\rm T}$ using a proton-proton (pp) reference measured at the same collision energy. The results are compatible with unity in the whole $p_{\rm T}$ range. The average of the non-strange D mesons $R_{\rm pPb}$ is compared with theoretical model predictions that include initial-state effects and parton transport model predictions. The $p_{\rm T}$ dependence of the D$^0$, D$^+$, and D$^{*+}$ nuclear modification factors is also reported in the interval $1< p_{\rm T} < 36$ GeV/$c$ as a function of the collision centrality, and the central-to-peripheral ratios are computed from the D-meson yields measured in different centrality classes. The results are further compared with charged-particle measurements and a similar trend is observed in all the centrality classes. The ratios of the $p_{\rm T}$-differential cross sections of D$^0$, D$^+$, D$^{*+}$, and D$^+_s$ mesons are also reported. The D$^+_s$ and D$^+$ yields are compared as a function of the charged-particle multiplicity for several $p_{\rm T}$ intervals. No modification in the relative abundances of the four species is observed with respect to pp collisions within the statistical and systematic uncertainties.

==> aliases.tex <==
\newcommand{\pp}{pp~}
\newcommand{\mpp}{\mathrm{pp}}
\newcommand{\sqrts}{\sqrt{s}}
\newcommand{\sqrtsNN}{\sqrt{s_{\scriptscriptstyle \rm NN}}}
\newcommand{\lsim}{\,{\buildrel < \over {_\sim}}\,}
\newcommand{\gsim}{\,{\buildrel > \over {_\sim}}\,}
\newcommand{\av}[1]{\left\langle #1 \right\rangle}
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\keV}{\mathrm{keV}}
\newcommand{\MeV}{\mathrm{MeV}}
\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\TeV}{\mathrm{TeV}}
\newcommand{\tev}{\mathrm{TeV}}
\newcommand{\ev}{\mathrm{eV}}
\newcommand{\kev}{\mathrm{keV}}
\newcommand{\mev}{\mathrm{MeV}}
\newcommand{\gev}{\mathrm{GeV}}
\newcommand{\gevc}{\mathrm{GeV}/c}
\newcommand {\massStyle}[1] {\mbox{\ensuremath{\text{#1}\kern-0.1em /\kern-0.12em c^2}}}
\newcommand {\mass}     {\massStyle{MeV}}
\newcommand {\kmass}    {\massStyle{keV}}
\newcommand {\mmass}    {\massStyle{MeV}}
\newcommand {\gmass}    {\massStyle{GeV}}
\newcommand{\fm}{\mathrm{fm}}
\newcommand{\mm}{\mathrm{mm}} 
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\m}{\mathrm{m}}
\newcommand{\mum}{\mathrm{\mu m}}
\newcommand{\s}{\mathrm{s}}
\newcommand{\ns}{\mathrm{ns}}
\newcommand{\mrad}{\mathrm{mrad}}
\newcommand{\mb}{\mathrm{mb}}
\newcommand{\mub}{\mathrm{\mu b}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\PbPb}{\mbox{Pb--Pb}}
\newcommand{\pPb}{\mbox{p--Pb}}
\newcommand{\AuAu}{\mbox{Au--Au}}
\newcommand{\IonIon}{\mbox{A--A}}
\newcommand{\pt}{p_{\rm T}}
\newcommand {\cTau}{\ensuremath{c.\tau}}
\newcommand{\dNdy}{{\rm d}N_{ch}/{\rm d}y}
\newcommand{\momwin}{[$p$, $p$+$\Delta$ $p$]}
\newcommand{\DtoKpi}{{\rm D}^0 \to {\rm K}^-\pi^+}
\newcommand{\DtoKpipi}{{\rm D}^+\to {\rm K}^-\pi^+\pi^+}
\newcommand{\DstartoDpi}{{\rm D}^{*+} \to {\rm D}^0 \pi^+}
\newcommand{\DstartoDpiPrecise}{{\rm D^{*+}(2010)\to D^0\pi^+}}
\newcommand{\Dzero}{{\rm D^0}}
\newcommand{\Ds}{{\rm D^+_s}}
\newcommand{\Dzerobar}{\overline{\rm D}{}^{0}}
\newcommand{\Dstar}{{\rm D^{*+}}}
\newcommand{\Dstarm}{{\rm D^{*-}}}
\newcommand{\DstarMDzero}{\mbox{($\Dstar - \Dzero$)}}
\newcommand{\Dplus}{{\rm D^+}}
\newcommand{\Dminus}{{\rm D^-}}
\newcommand{\Jpsi}{{\rm J}/\psi}

\newcommand{\piZero}        {\mbox{$\mathrm {\pi^0}$}}
\newcommand{\piMinus}       {\mbox{$\mathrm {\pi^-}$}}
\newcommand{\piPlus}        {\mbox{$\mathrm {\pi^+}$}}
\newcommand{\piPlusMinus}   {\mbox{$\mathrm {\pi^{\pm}}$}}
\newcommand{\Kzs}       {\mbox{$\mathrm {K^0_S}$}}
\newcommand{\Kminus}    {\mbox{$\mathrm {K^-}$}}
\newcommand{\Kplus}     {\mbox{$\mathrm {K^+}$}}
\newcommand{\Kplusmin}  {\mbox{$\mathrm {K^{\pm}}$}}
\newcommand{\rmKstar}    {\mbox{$\mathrm{K}^*\mathrm{(892)}^0$}}
\newcommand{\rmPhiMes}    {\mbox{$\mathrm {\phi(1020)}$}}
\newcommand{\rmB}           {\mbox{$\mathrm {B}$}}
\newcommand{\rmBzero}       {\mbox{$\mathrm {B^{0}}$}}
\newcommand{\rmBplus}       {\mbox{$\mathrm {B^{+}}$}}
\newcommand{\rmBminus}      {\mbox{$\mathrm {B^{-}}$}}
\newcommand{\rmBplusMinus}  {\mbox{$\mathrm {B^{\pm}}$}}
\newcommand{\rmBzeroS}      {\mbox{$\mathrm {B^{0}_s}$}}
\newcommand{\rmLambdaB} {\mbox{$\mathrm {\Lambda}_{b}^{0}$}}



\newcommand{\ccbar}{${\rm c}\bar{\rm c}$~}
\newcommand{\nbinv}{{\rm nb^{-1}}}
\newcommand{\decleng}{{\rm L}_{xyz}}
\newcommand{\dEdx}{{\rm d}E/{\rm d}x}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\cubar}{{\rm c}\bar{\rm u}}
\newcommand{\cdbar}{{\rm c}\bar{\rm d}}
\newcommand{\mur}{\mu_{\rm R}}
\newcommand{\muf}{\mu_{\rm F}}
\newcommand{\mc}{m_{\rm c}}
\newcommand{\sigmatot}{\sigma_{\rm tot}}
\renewcommand{\PbPb}{\mbox{Pb--Pb}}
\newcommand{\Npart}{N_{\rm part}}
\newcommand{\Ncoll}{N_{\rm coll}}
\newcommand{\Raa}{R_{\rm AA}}
\newcommand{\RpPb}{R_{\rm pPb}}
\newcommand{\RAA}{R_{\rm AA}}
\newcommand{\TAA}{T_{\rm AA}}
\newcommand{\RCP}{R_{\rm CP}}
\newcommand{\meanpt}{{\langle p_{ {\mathrm T} } \rangle}}
\newcommand{\QpPb}{\ensuremath{Q_\mathrm{pPb}}}
\newcommand{\Qcp}{\ensuremath{Q_\mathrm{CP}}}
\newcommand{\TpPb}{\ensuremath{T_\mathrm{pPb}}}
\newcommand{\QpPbmult}{\ensuremath{Q_\mathrm{pPb}^\mathrm{mult}}}
\newcommand{\TpPbmult}{\ensuremath{T_\mathrm{pPb}^\mathrm{mult}}}
\newcommand{\Ncollmult}{\ensuremath{N_{\rm coll}^\mathrm{mult}}}
\newcommand{\Npartmult}{\ensuremath{N_{\rm part}^\mathrm{mult}}}
%\newcommand{\Lint}{{\cal{L}}_{\mathrm{int}}}
\newcommand{\Lint}{{L}_{\mathrm{int}}}
\newcommand{\fprompt}{\ensuremath{f_{\rm prompt}}}


\newcommand{\Ntrk}{N_{\rm tracklets}}
\newcommand{\Nch}{N_{\rm ch}}
\newcommand{\zvtx}{z_{\rm vtx}}
\newcommand{\dNdEta}{{\rm d}N_{\rm ch}/{\rm d}\eta}


